MYCROFT: Towards Effective and Efficient External Data Augmentation

Machine learning (ML) models often require large amounts of data to perform well. When the available data is limited, model trainers may need to acquire more data from external sources. Often, useful data is held by private entities who are hesitant to share their data due to propriety and privacy concerns. This makes it challenging and expensive for model trainers to acquire the data they need to improve model performance. To address this challenge, we propose Mycroft, a data-efficient method that enables model trainers to evaluate the relative utility of different data sources while working with a constrained data-sharing budget. By leveraging feature space distances and gradient matching, Mycroft identifies small but informative data subsets from each owner, allowing model trainers to maximize performance with minimal data exposure. Experimental results across four tasks in two domains show that Mycroft converges rapidly to the performance of the full-information baseline, where all data is shared. Moreover, Mycroft is robust to noise and can effectively rank data owners by utility. Mycroft can pave the way for democratized training of high performance ML models.

==> sections/motivation.tex <==
In this section, we motivate the need for our proposed framework \method~that
enables model trainers to find data owners with relevant data in a
data-efficient manner. We then present the formal setup for the external data
augmentation problem.

\subsection{Why perform external data augmentation?}
In this section, we examine the conditions under which external data
augmentation is necessary for model trainers. We note that while there is
related work on obtaining data in from data marketplaces, most of this work
focuses on data acquisition in the case when the model trainer is starting from
scratch.

\noindent \textbf{Limited data availability for individual model trainers:}
Recent successes in training performant ML models have largely been driven by
the availability of large amounts of data. However, these models have been
developed by entities with considerable resources to pay contractors to obtain
and label data for them. Most individuals or small institutions struggle to
obtain the requisite data to train performant ML models, particularly in domains
where large open-source models and datasets do not already exist. It can be
challenging to obtain data which is demographically diverse due to hesitancy on
the part of individuals to part with their data. It is also difficult to obtain
discrete datasets that have good coverage of the input space, with years of
research required to create datasets such as LAION for the extremely popular
task of image captioning.~\van{other reasons include entities have constraints such as
geography, budget and time. Or when some data is extremely rare because those are uncommon events like rare diseases or earthquakes.} 
In addition, it is challenging to set up federated
learning by involving a sufficient number of stakeholders, although it can
provide privacy-preserving access to diverse data.~\van{I think the last sentence 
should be one motivation on its own} 


\noindent \textbf{Changing conditions at test time:} When the model trainer
deploys their model, they may find poor performance due to data drift. Acquiring
more data is critical to counter data drift, but there are numerous reasons why
the model trainer may not be able to acquire the data themselves, including lack
of access to the right data sources or lack of resources. In such cases, the
model trainer will prefer to perform \problem, particularly if they are aware
that \dataowners~with relevant data exist.~\van{What is the difference between this and the previous motivation?}






\van{\textbf{High cost while limited confidence in model improvement of other sharing mechanisms:}}
There are various ways where an external entity can help another entity to improve their models.
These includes various methods such as data sharing, federated learning, model sharing or weight sharing of features. 
Model sharing is a method where one entity shares their model with another entity. 
One limitation of this approach is that it assumes the model working well on one entity would likely work well for another entity.
However, this is not always the case, for example, a model trained to predict anomalous traffic in one network might not 
work well for another network since the traffic patterns might be different. The same is true for weight sharing methods. On the other hand,
although federated learning can provide privacy-preserving access to diverse data, it is challenging to set up federated learning due to various 
requiresments for stakeholders such as requiring them all to train simultenously using the same model. Data owners might not want to train their 
models again especially if their models are already good enough and it is computationly expensive to train the model again. 
Therefore, without a clear demonstration of data utility, initiating these collaborative model improvement strategies might 
incur high costs with uncertain benefits for the model trainers.


\van{\textbf{Promising impact of using external data augmentation:}}

External data augmentation has show many promising results in improving model performance.
\van{Zain, please add the section SOTA on image net is actually using external noisy data}
The key idea behind the improvement of the model is that external data might provide a 
range of scenarios and examples are are not present or underrepresented in the model, 
allowing the model to have a better representation for the missing data. In addition, when the training data of 
the model trainer is outdated, augmenting the training data with more recent data from external sources can allow
the model to be up to date with the latest trends and changes in the data. Additionally, it can be a cost-effective solution
for many entities where the cost of acquiring data from external sources is much lower than the cost of collecting their own data. 
Finally, compared to other methods such as model sharing or federated learning, external data augmentation is a more flexible method
where the model trainer can use the data to train their own model and have full control over the model training process. It also
allow the model trainers to have more confidence in the quality of the data from external sources since they can evaluate such data.




\subsection{Challenges of external data augmentation}
\van{\textbf{Challenges of data augmentation:}} Although external data
augmentation is very promising in solving problems mentioned above, there are
challenges hindering its adoption.~(i) Finding the data owners that have the
relevant data is an expensive and challenging tasks. There might be many data
owners potentially possess the data that is needed. If we are to check all of
these data owners or all of the data that each data owners have, it would be
very expensive and time-consuming. For example, if you want to improve your
model of dog predictions, there may be many data owners possess data about
dogs. However, it is still unknown whether they have images about specific dog
breeds that your model is not performing well on.  
(ii) Model trainers do not have the resources to acquire too much data due to
limited budget, communication cost to acquire data, and limited computation
power to train on too much data.\@ (iii) Data owners might be unwilling to share a
lot of data that they have due to privacy concerns. They might also be unwilling
to spend resources working collaboratingly with data owners before establishing
a data sharing contract.\@ (iv) Too much irrelevant data can negatively impact
model performance while incurring high computation cost for training the model.
This is especially when data owners' data can be very diverse. The data that the
model trainer need can be a very small subset of the data that the data owner
has.

Given these reasons, it is crucial to have an effective and efficient data
sharing method that (i) Help data owners find the smallest useful samples to
allow model trainers to test the utility of the data before acquiring all of the
data.\@ (ii) Does not require data owners to spend too much resources looking for
the relevant data or  working collaboratively with the model trainer before
establishing a data sharing contract.\@ (iii) Help model trainers narrow down the
most useful subset of useful data for augmentation.





\subsection{Problem Setting}

We consider a setting where there is a model trainer (\MT) and $m$ data
owners (\DOs), where $m$ is an integer $\geq 1$. \MT~has trained a model $M_{\text{MT}}$ on its own dataset
$D_{\text{MT}}$ and is aiming to improve their performance (or lower their loss)
on test data $D_{\text{test}}$ via \problem. The performance of \MT's model on
$D_{\text{test}}$ is measured with respect to a task $T$. For simplicity, we
will assume that the task is supervised learning, so the performance is measured
as 
\begin{align}
    L(D_{\text{test}},M) = \sum_{z_i \in D_{\text{test}}} \ell_T(y_i,M(x_i)).
\end{align}

Each \DO~has a dataset $D_i$ which could aid \MT~in improving their performance
on the test set. However, due to concerns such as data privacy and economic
considerations, they are unwilling to share all of their data directly with \MT~so 
that \MT~can evaluate its effectiveness. Rather, they aim to provide \MT~with
a small subset of their data that establishes the utility of their full dataset
$D_i$ and can then convince \MT~to enter into a well-defined data sharing
agreement. The task for each \DO~is then:

\begin{definition}[Task for each \DO]
    Find the smallest $ D_{\text{useful}} \subseteq D_i $ such that $
    L(\Dhard,M') \leq L(\Dhard,M_{\text{MT}}) $, where $M_{\text{MT}} =
    \train(D_{\text{MT}})$ and $M_{\text{MT}}' = \train(D_{\text{MT}} \cup
    D_{\text{useful}})$.
\end{definition}

We operate within the following design choices to define the setting
in which we investigate data sharing between \MT~and the \DOs:
\begin{enumerate}[start=1,label={\bfseries DC.\arabic*}]
    \item There exists a subset $\Dhard \subseteq D_{\text{test}}$ with accurate
    ground-truth labels on which $M_{\text{MT}}$ performs poorly, which \MT~communicates to the \DOs.\label{c1}
    \item \MT~does not share $M_{\text{MT}}$ with the \DOs.\label{c2}
    \item No \DO~is willing to share their full training data with \MT~to help
    them improve their performance on $\Dhard$.\label{c3}
    \item Each participating \DO~has samples from at least one of the classes
    contained within $\Dhard$.\label{c4}
\end{enumerate}

To address~\ref{c1}, \MT~requests data from the \DOs~in order to determine which
\DO's data will be the most useful for their task. We assume that \MT~shares 
the difficult subset $\Dhard$ with the \DOs. Without knowledge of the
difficult subset, the \DOs~cannot share data that would help in a meaningful
manner, and would simply be guessing at what data would be useful. Further, if
$\Dhard$ is incorrectly labeled, the \DOs~cannot evaluate if their local model
is relevant to the provided samples.

In~\ref{c2}, we do not assume that the \DOs~have access to $M_{\text{MT}}$ as it is unlikely
the model trainer will be willing to share their local model for intellectual
property and privacy reasons. While this makes the task more challenging for
each \DO~to solve, in \cref{sec: evaluation}, we show that even without access to $M_{\text{MT}}$,
the \DOs~are able to share useful data.

Common-sense privacy and economic concerns guide~\ref{c3} as a \DO~will aim to
address by providing just enough data for \MT~to be convinced of the utility of
their data. After utility is established, \MT~may enter into an agreement with
the best \DO(s) for its purposes.If the \DOs~were willing to share all of their
data, then \MT~could simply locally evaluate which \DO~is the best. This
approach, which we refer to as \fullinfo, provides an upper bound
on the improvement in performance that \MT~can get by using data from a single
\DO~in conjunction with $D_{\text{MT}}$. We compare the performance of our
methods to it in \cref{sec: evaluation}.~\ref{c4} just rules out \DOs~with no
relevant data to the task under consideration.

\arjun{Say what we are not considering}
% In addition, \MT needs to determine,
% from these data summaries, which of the data owners has the most useful data,
% while reducing its local computation. We explore methods for \MT to do this in
% \cref{subsec:computational_speed_ups}.







==> tables/checklist.tex <==
\begin{enumerate}

\pagebreak


\section*{NeurIPS Paper Checklist}

    \item {\bf Claims}
        \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: The abstract and introduction clearly state the contribution of the paper. Section \ref{sec: methods} describes the proposed method, and Section \ref{subsec: exp_setup} presents the experimental results that support the claims made in the abstract and introduction.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
            \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
            \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
            \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
        \end{itemize}
    
    \item {\bf Limitations}
        \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Section \ref{sec: discussion} discusses the limitations of the proposed method and the experimental results and describes the computer efficiency of the proposed algorithms in Section \ref{subsec: ablation} and Appendix \ref{appsec:runtime_analysis}
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
            \item The authors are encouraged to create a separate "Limitations" section in their paper.
            \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
            \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
            \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
            \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
            \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
            \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
        \end{itemize}
    
    \item {\bf Theory Assumptions and Proofs}
        \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Assumptions are stated in Section \ref{subsec: notation} and the proofs are provided in Appendix \ref{appsec:proofs}.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not include theoretical results. 
            \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
            \item All assumptions should be clearly stated or referenced in the statement of any theorems.
            \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
            \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
            \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
        \end{itemize}
    
        \item {\bf Experimental Result Reproducibility}
        \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: All experimental details are provided in Section \label{subsec: exp_setup} and the supplemental material. The paper also attach the source code and data to the submission.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not include experiments.
            \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
            \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
            \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
            \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
            \begin{enumerate}
                \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
                \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
                \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
                \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
            \end{enumerate}
        \end{itemize}
    
    
    \item {\bf Open access to data and code}
        \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
        \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: We attach our code and data used to the submission
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that paper does not include experiments requiring code.
            \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
            \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
            \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
            \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
            \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
            \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
            \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
        \end{itemize}
    
    
    \item {\bf Experimental Setting/Details}
        \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: We describe the training details and models used in Section \ref{subsec: exp_setup} and Appendix \ref{appsec:training_details}
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not include experiments.
            \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
            \item The full details can be provided either with the code, in appendix, or as supplemental material.
        \end{itemize}
    
    \item {\bf Experiment Statistical Significance}
        \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
        \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Due to the computational expenses and the number of experiments done, we did not perform statistical significance tests.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not include experiments.
            \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
            \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
            \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
            \item The assumptions made should be given (e.g., Normally distributed errors).
            \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
            \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
            \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
            \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
        \end{itemize}
    
    \item {\bf Experiments Compute Resources}
        \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: 
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not include experiments.
            \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
            \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
            \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
        \end{itemize}
        
    \item {\bf Code Of Ethics}
        \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Yes we do not conduct study that involves a human subject. We also use public dataset that do not have any harms to the society.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
            \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
            \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
        \end{itemize}
    
    
    \item {\bf Broader Impacts}
        \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: The paper discusses the potential societal impacts of the work performed in Section \ref{sec: discussion}.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that there is no societal impact of the work performed.
            \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
            \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
            \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
            \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
            \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
        \end{itemize}
        
    \item {\bf Safeguards}
        \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
        \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Our study does not involve any models or data that have high risk for misuse
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper poses no such risks.
            \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
            \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
            \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
        \end{itemize}
    
    \item {\bf Licenses for existing assets}
        \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: We properly credit all creators of the assets in our paper.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not use existing assets.
            \item The authors should cite the original paper that produced the code package or dataset.
            \item The authors should state which version of the asset is used and, if possible, include a URL.
            \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
            \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
            \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
            \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
            \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
        \end{itemize}
    
    \item {\bf New Assets}
        \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
        \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: We have description about the new assets in \ref{appsec:dataset_details}
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not release new assets.
            \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
            \item The paper should discuss whether and how consent was obtained from people whose asset is used.
            \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
        \end{itemize}
    
    \item {\bf Crowdsourcing and Research with Human Subjects}
        \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
        \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Our study does not involve Human Subjects or Crowdsourcing.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
            \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
            \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
        \end{itemize}
    
    \item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
        \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
        \item[] Answer: \answerNA{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
        \item[] Justification: Our study does not involve Human Subjects.
        \item[] Guidelines:
        \begin{itemize}
            \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
            \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
            \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
            \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
        \end{itemize}
    
    \end{enumerate}
    
    
   

==> tables/do_types_dvw.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|}
    \hline
    DO Type & Description \\
    \hline
    DO-1 & Many Dogs-vs-Wolves-Hard \\
    \hline
    DO-2 & Few Dogs-vs-Wolves-Hard \\
    \hline
    DO-3 & Many Dogs \& Wolves with no background \\
    \hline
    DO-4 & Many Noisy Dogs-vs-Wolves-Hard \\
    \hline
    DO-5 & Many Dogs-vs-Wolves-Easy \\
    \hline
    DO-6 & Many Dogs \& Wolves from Imagenet \\
    \hline
    \end{tabular}
    \caption{Types of DOs in the Dogs vs Wolves experiment.}
    \label{tab:do_types_dvw}
    
\end{table}

==> tables/dvw_results.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    DO Type & \randsamp & Similarity sampling & Gradient Matching & \fullinfo \\
    \hline
    DO-1 & - & 49.8 & 51.3 & 86 \\
    \hline
    DO-2 & - & 39.6 & 46 & 71.3 \\
    \hline
    DO-3 & - & 26.7 & 31.6 & - \\
    \hline
    DO-4 & - & 37.5 & 47 & - \\
    \hline
    DO-5 & - & 24.2 & 29.6 & 33.3 \\
    \hline
    DO-6 & - & 38.7 & 40.5 & - \\
    \hline

    \end{tabular}

\caption{Results for $\Dhard$ after \MT retrains their model with each \DO's data using different external data augmentation techniques on the Dogs \& Wolves dataset.}
\label{tab: dvw_results}

\end{table}    

==> tables/enola_vs_random_scenarios.tex <==

\resizebox{1.0\textwidth}{!}{ 
\begin{tabular}{ccccc}
    
    \toprule
    & \multicolumn{2}{c}{Corrupted Data} & \multicolumn{2}{c}{Corrupted Labels} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}
    Dataset &\method & \makecell{\texttt{random}-\\ \texttt{sampling}}  & \method &\makecell{\texttt{random}-\\ \texttt{sampling}} \\
     \midrule
    Food-101 - UPMC  & 55 & 30 & 55 & 32.5 \\

    Food-101 - ISIA500  & 55 & 32.5 & 57.5 & 35 \\

    Imagenet - Tsinghua & 61.5 & 37.5 & 61.5 & 25 \\

    \makecell{\dvwS - \\ \dvwN} & 75 & 18.8 & 75 & 18 \\
    \bottomrule
  \end{tabular}
}
  %\caption{Accuracy of $M_{\text{MT}}'$ when tested on $\Dhard$ when trained on data selected by \method versus by random sampling. $\Dhard$= 4/class, $D^{\text{useful}}$ = 16/class.}\label{tab:enola_vs_random_scenarios}










%% For nicer table formatting
%\begin{table}
%  \centering
%  \begin{tabular}{|c|c|c|c|c|c|c|}
%    \hline
%    Dataset & \multicolumn{2}{c|}{\makecell{Generic Data \\ Augmentation}} & \multicolumn{2}{c|}{Corrupted Data} & \multicolumn{2}{c|}{Corrupted Labels} \\
 %   \hline
 %   & \method & \makecell{Random \\sampling} &\method & \makecell{Random \\sampling}  & \method & \makecell{Random \\sampling} \\
 %   \hline
 %   Dogs \& Wolves & 81.3 & 20 & 75 & 18.8 & 75 & 18 \\
 %   \hline
 %   Food-101 - UPMC & 55 & 40 & 55 & 30 & 55 & 32.5 \\
 %   \hline
 %   Food-101 - ISIA500 & 55\ & 40 & 55 & 32.5 & 57.5 & 35 \\
 %   \hline
 %   Imagenet - Tsinghua & 65 & 50 & 62.5 & 37.5 & 62.5 & 25 \\
 %   \hline
  %\end{tabular}
  %\caption{Accuracy of $M_{\text{MT}}'$ when tested on $\Dhard$ when trained on data selected by \method versus by random sampling. $\Dhard$= 4/class, %$D^{\text{useful}}$ = 16/class.}\label{tab:enola_vs_random_scenarios}
%\end{table}


==> tables/finetune_v_retrain.tex <==
%\begin{table}[ht]
%    \centering
%    \begin{tabular}{|c|c|c|}
%    \hline
%    Technique & Dogs \& Wolves & ISIA-500 \\
%    \hline
%    Finetune  & 87.5 & 55  \\
%    \hline
%    Retrain  & 87.5 &  41.5 \\
%    \hline
%    \end{tabular}
%    \caption{Comparison of accuracy of $M_{\text{\MT}}'$ on $\Dhard$ when $MT$ chooses to retrain or finetune their model with 
%    $\Duseful$ on the Dogs \& Wolves and ISIA-500 datasets. }\label{tab :finetune_v_retrain} 
%\end{table}    


\begin{table}[ht]
\resizebox{.55\textwidth}{!}{
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Technique & UPMC-101 &  ISIA-500 & Tsinghua  & Dogs \& Wolves \\
\hline
Finetune & 55 & 55  & 61.5 & 87.5  \\
\hline
Retrain  & 0 & 50  &  0 &  87.5 \\
\hline
\end{tabular}  
}  
\caption{Comparison of accuracy of $M_{\text{\MT}}'$ on $\Dhard$ when $MT$ chooses to retrain or finetune their model with $\Duseful$.}\label{tab :finetune_v_retrain} 

\end{table}





==> tables/symbols_table.tex <==
\begin{table}[ht]
   
    \begin{tabular}{|c|c|}
    \hline
    Symbol & Description \\
    \hline
    $\DO$ & Data Owner. \\
    \hline
    $\MT$ & Model Trainer. \\
    \hline
    $D_{\text{MT}}$ & \MT's dataset \\
    \hline
    $M_{\text{MT}}$ & Model of the \MT. \\
    \hline
    $D_{\text{test}}$ & \MT's test dataset. \\
    \hline
    $ D_{\text{useful}} $ & Data subset of \DO that is likely useful for \MT  \\
    \hline
    $\Dhard$ & The dataset that \MT~has access to. \\
    \hline
    \end{tabular}    
    \caption{Table of notations used in the paper.} \label{tab:notations}
    
\end{table}
    

==> tables/unicom_v_l2.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Retrieval space & Dogs \& Wolves & Other \\
    \hline
    Unicom  & 74 & 26  \\
    \hline
    \makecell{ResNet50}  & 6 & 94  \\
    \hline
    \end{tabular}
\caption{Comparison of Unicom with a retriever based on l2 distances in the
feature space of ResNet50 \arjun{just mention in text}}\label{tab :unicom_ablation} 
\end{table}    



